Platform Competition in the Autobidding World

We study the problem of auction design for advertising platforms that face strategic advertisers who are bidding across platforms. Each advertiser's goal is to maximize their total value or conversions while satisfying some constraint(s) across all the platforms they participates in. In this paper, we focus on advertisers with return-over-investment (henceforth, ROI) constraints, i.e. each advertiser is trying to maximize value while making sure that their ROI across all platforms is no less than some target value. An advertiser interacts with the platforms through autobidders -- for each platform, the advertiser strategically chooses a target ROI to report to the platform's autobidder, which in turn uses a uniform bid multiplier to bid on the advertiser's behalf on the queries owned by the given platform. Our main result is that for a platform trying to maximize revenue, competition with other platforms is a key factor to consider when designing their auction. While first-price auctions are optimal (for both revenue and welfare) in the absence of competition, this no longer holds true in multi-platform settings. We show that there exists a large class of advertiser valuations over queries such that, from the platform's perspective, running a second price auction dominates running a first price auction. Furthermore, our analysis reveals the key factors influencing platform choice of auction format: (i) intensity of competition among advertisers, (ii) sensitivity of bid landscapes to an auction change (driven by advertiser sensitivity to price changes), and (iii) relative inefficiency of second-price auctions compared to first-price auctions.

==> introduction.tex <==
\section{Introduction}

%In recent years, there has been a significant increase in the number of advertisers who use automated bidders (henceforth, auto-bidders) to submit bids for them in advertisement auctions. 


Consider the problems that both an online advertisement platform and online advertisers face every day when participating in millions of ad auctions. The platform's problem is to design an auction format that is attractive to advertisers and has strong revenue guarantees. Given such an auction format, the advertisers' problem is to compute optimal bids to maximize an objective function. Let's delve into each of these problems more carefully. 

How should a platform choose an auction format to auction off their queries? Whatever format it chooses will have a repercussion on how the advertisers will bid, and this in turn affects both efficiency and revenue. For example, under a truthful auction the platform can expect bids to be more aggressive and allocations to be more efficient than under a non-truthful auction. How this decision ultimately impacts revenue and efficiency will depend on the particular equilibrium advertisers settle on. Thus in order to correctly predict which auction format will be more profitable, the platform must understand the possible equilibrium the advertisers will settle on given a format. 

On the other hand, the advertisers problem is to compute bids that optimize their objectives given the auction format that the platform has chosen while taking into account the decisions competing advertisers will make.  Due to the scale and frequency of this problem, it is common for platforms to provide advertisers with the option of using an automated bidder, a program which takes into account the advertisers' objective and values for queries and submits optimal bids on their behalf. 

A particularly common assumption on classical auction design literature is that the advertiser's objective is to maximize their profit. That is, advertiser's are modeled as to maximize the difference between the value of the queries they get and their cost. Profit-maximization is theoretically elegant and well understood. One advantage of profit-maximizing as a model is that it makes bidding across different queries independent. For the sake of the argument, suppose that the advertiser knew in advance how much it would cost to win any query. However much an advertiser is willing to pay for one query has no impact on how much they are willing to pay for a different query. The advertiser will bid minimally to win any query where their value exceeds the cost, and bid below the cost otherwise. Moreover, a change in the price of a query will not affect the bid on a different query.    

In recent years, due to the rise of auto-bidders, there has been a shift in this modelling assumption. Practitioners and advertisers favor a model where rather than trying to maximize their profit, advertisers try to maximize their value for the queries won. Naturally, there must be some constraint to keep the advertiser from bidding unreasonably to win every possible query. One way to do this is to assume that each advertiser has a target average return on investment of $T$. Hence in this value-maximizing model the advertiser is trying to maximize the value of the queries they win subject to their total cost being no more than $T$ times the their total value. In this model we no longer have the independence property from the profit-maximizing model. Suppose again that the advertiser knew in advance how much it would cost to win a query. After finding their carefully computed optimal bids, a change in price for a query could affect how much the advertiser is willing to bid on other queries. For example, if a query became substantially cheaper, this gives the advertiser more slack in their target constraint to apply on other more expensive queries. 

At this point we can present a description of the platform-advertiser game. 

\begin{enumerate}
    \item The platform announces an auction format $a \in \mathcal{A}$. 
    \item Advertiser $i$ computes their optimal bid vector $\vec{\mu}_i(a)$. 
    \item Queries are allocated and payoffs are accrued. 
\end{enumerate}

To find an equilibrium of this game, the platform needs to compute the equilibrium bids advertisers will submit for every auction format $a$ they are considering. Then they can compute the revenue-maximizing auction format. This means that to describe an equilibrium we need $|\mathcal{A}| \cdot n$ vectors, where $n$ is the number of advertisers (and the dimension of the vectors is the number of queries). Previous work shows that if there is a single platform facing multiple value-maximizing advertisers, the problem becomes rather simple. It is in both the platform's and advertisers' best interest for the platform to use a First Price Auction and for the advertisers to bid truthfully. This maximizes both the overall advertisers' efficiency and the platforms revenue. This result is stunning as it suggests a simple, transparent solution to a seemingly multi-dimensional, sequential problem. The aim of this paper is to investigate if the same conclusion holds in the presence of \emph{multiple} competing revenue-maximizing platforms. This changes the game description slightly, but substantially increases the description complexity of an equilibrium. 

\begin{enumerate}
    \item The platforms simultaneously announce their auction format, encoded by a vector $\vec{a} \in \mathcal{A}^m$. 
    \item Advertiser $i$ computes their optimal bid vector $\vec{\mu}_{i,j}(\vec{a})$ for platform $j$. 
    \item Queries are allocated and payoffs are accrued. 
\end{enumerate}

If there are $m$ platforms, then in order to describe an equilibrium a platform needs to compute $m \cdot n \cdot |\mathcal{A}|^m$ vectors, where $m$ is the number of platforms. Moreover, a platform can no longer choose a unilaterally revenue-maximizing auction format. The ultimate outcome will be the equilibrium of the game played between the platforms. We can simplify the problem by forcing advertisers to use a fixed bid multiplier on a given platform or on all platforms. We refer to the former as the non-uniform bid multiplier setting and the latter as the uniform bid multiplier setting.  

We will first consider the case of uniform bid multipliers, and show that in that case the results from the single-platform case still hold. 

\begin{theorem}
In the case of multiple platforms and multiple value-maximizing advertisers subject to uniform bid multipliers, the unique Nash equilibrium of the platform-advertiser game is for the platforms to use First Price Auction and for advertisers to bid truthfully.  
\end{theorem}

We then consider the single-bidder, multi-platform case with non-uniform bidding and again show that the single-platform case results holds. 

\begin{theorem}
In the case of multiple platforms and a single value-maximizing advertisers subject to non-uniform bid multipliers facing a static price landscape, the unique Nash equilibrium of the platform-advertiser game is for the platforms to use First Price Auction and for advertiser to bid truthfully.  
\end{theorem}

Most of our attention on the case of two revenue-maximizing, competing platforms and two strategic advertisers subject to non-uniform bid multipliers facing an otherwise static price landscape. Moreover, we even restrict the space of auctions the platforms can use to the two canonical auction formats: First Price and Second Price Auction. As it turns out, this almost minimal extension of the single-platform setting suffices to show that the conclusion of the single-platform case may not universally hold in the multi-platform case.  

\begin{theorem}
In the case of two platforms running either First Price or Second Price Auction and a two value-maximizing advertisers subject to non-uniform bid multipliers facing a static price landscape, there are broad families of instances where it is not an equilibrium for the platforms to use the First Price Auction. In fact, there are cases where Second Price Auction is a dominant strategy. 
\end{theorem}

The main conclusion of this paper is that the wisdom from the single-platform case may not hold in the case of multiple platforms: there exist broad classes of reasonable settings where First Price is not the equilirbium that platforms will land on. We provide multiple examples of the Theorem above, studying instances where the advertisers' valuations are positively correlated, negatively correlated or not correlated at all. We also introduce some axis of symmetry to help shed light on our results. 

INSERT MAIN TAKEAWAYS HERE? 

\begin{comment}
\subsection{Related Works}

\subsection{Our Contributions}

\subsubsection{Organization of this paper}
\end{comment}


==> non_uniform_bidding_symmetric.tex <==
\section{Missing Proofs from Section~\ref{sec:inefficiency_free} }\label{sec:proof_inefficiency_free}


%Mingfei:
%Solve the game as general as possible where bidder 1 has value %$v_1(q) = v(q)$ increasing differenable, and $v_2(q) = v(1-q)$.
%Ideally solve the case where for platform 1, valuations are $(\gamma v_1(q), \gamma v_2(q))$ and platform 2 has valuations 
%$((1-\gamma) v_1(q), (1-\gamma) v_2(q))$. W 

%What conditions are such that $SPA,SPA$ is equilibrium. 

%\mingfeinote{TODO: Verify landscape convexity: If $v(\cdot)$ is concave, then marginal is increasing.}

%In this section we study the setting where there are two advertisers with inverted valuations. More specifically, let $v(q)$ be any non-decreasing, differentiable function. Advertiser 1 has value function $v_1(q)=v(q)$ and advertiser 2 has value function $v_2(q)=v(1-q)$. Let $\gamma\in (0,1)$ be the market share of platform 1. Advertisers have value $(\gamma v_1(q), \gamma v_2(q))$ for platform 1 and $((1-\gamma) v_1(q), (1-\gamma) v_2(q))$ for platform 2.

For the remaining of the section, we study the equilibrium of the game. We begin with the setting of two platforms with asymmetric market share. We denote $\gamma\in [0,1]$ the market share of platform $1$ (so the market share of platform $2$ is $1-\gamma$).

\subsection{Two Platforms with Asymmetric Market Share}\label{subsec:mirror_two_platform}

We will compute the advertisers' equilibrium and the platforms' revenue for each profile of the 2-player game between platforms. For ease of notation let $L=\int_{0}^{1/2} v(q)dq$ and $H=\int_{1/2}^1 v(q)dq$.

\paragraph{Case 1: (FPA, FPA)} We know that advertisers will set multipliers $\mu_{ij} = 1$. In both platforms, advertiser 1 wins the query when $v(q)\geq v(1-q)$, i.e. $q\geq \frac{1}{2}$ since $v(\cdot)$ is non-decreasing. Now the revenue of platform 1 is $\int_0^{1/2}\gamma v_2(q)dq+\int_{1/2}^1\gamma v_1(q)dq=2\gamma \cdot H$. Similarly the revenue of platform 2 is $2(1-\gamma)\cdot H$.

\paragraph{Case 2: (SPA, SPA)} Now both advertisers will set the multipliers such that the payment meets their target, i.e. $\gamma\int_{\frac{1}{2}}^1 \mu v_2(q)dq+(1-\gamma)\int_{\frac{1}{2}}^1 \mu v_2(q)dq = \gamma\int_{\frac{1}{2}}^1 \mu v_1(q)dq+(1-\gamma)\int_{\frac{1}{2}}^1 \mu v_1(q)dq \Longleftrightarrow \mu = H/L$.
The revenue is $\gamma\int_{\frac{1}{2}}^1 \mu v_2(q)dq+\gamma\int_0^{\frac{1}{2}} \mu v_1(q)dq = 2\gamma \cdot H$ for platform 1. Similarly the revenue of platform 2 is $2(1-\gamma)\cdot H$.

\paragraph{Case 3: (SPA, FPA)} Denote $\mu_1^F, \mu_1^S$ the bid multipliers for advertiser 1 and $\mu_2^F, \mu_2^S$ the multipliers for advertiser 2 on the SPA, FPA platforms respectively. Then by \Cref{theo:spa_fpa__subgame} the following equations are satisfied:

\begin{enumerate}
    \item Target constraint for advertiser 1: $\int_{q_S}^1\mu_2^S\gamma v_2(q)dq + \int_{q_F}^1\mu_1^F(1-\gamma)v_1(q)dq = \int_{q_S}^1\gamma v_1(q)dq + \int_{q_F}^1 (1-\gamma)v_1(q)dq$
    \item Target constraint for advertiser 2:
    $\int_{0}^{q_S}\mu_1^S\gamma v_1(q)dq + \int_0^{q_F}\mu_2^F(1-\gamma)v_2(q)dq = \int_0^{q_S}\gamma v_2(q)dq + \int_{0}^{q_F} (1-\gamma)v_2(q)dq$
    \item Equalizing marginals for advertiser 1: $\frac{\mu_1^S}{\mu_1^F} = 1+\frac{\eta_1(q_F)+\eta_2(q_F)}{\gamma v_1(q_F)}\int_{q_F}^1\gamma v_1(q)dq$.
    \item Equalizing marginals for advertiser 2: $\frac{\mu_2^S}{\mu_2^F} = 1+\frac{\eta_1(q_F)+\eta_2(q_F)}{(1-\gamma) v_2(q_F)}\int_0^{q_F}(1-\gamma) v_2(q)dq$.
\end{enumerate}

Given the setting, it is natural to seek for a symmetric Nash equilibrium. 

\begin{lemma}\label{lem:sym:spfp}
There exists a symmetric Nash equilibrium for the advertisers in the (SPA, FPA) profile such that $\mu_1^S=\mu_2^S=\mu^S, \mu_1^F=\mu_2^F=\mu^F$ where
\begin{itemize}
    \item $\frac{\mu^S}{\mu^F}=1+\frac{2v'(1/2)}{v^2(1/2)}\cdot H,$
    \item $\mu^S \gamma L+\mu^F (1-\gamma) H = H.$
\end{itemize}
\end{lemma}
\begin{proof}
In any symmetric equilibrium, we must have that $q_F = q_S = 1/2$ since $\mu_1^S=\mu_2^S, \mu_1^F=\mu_2^F$. Since $v(\cdot)$ is non-decreasing, $\eta_1(q_F)=|\frac{v_1'(q_F)}{v_1(q_F)}|=\frac{v'(q_F)}{v(q_F)}$ and $\eta_2(q_F)=|\frac{v_2'(q_F)}{v_2(q_F)}|=\frac{v'(1-q_F)}{v(1-q_F)}$. Using the fact that $v_1(q)=v(q)$ and $v_2(q)=v(1-q)$, we have that the target constraints for both advertisers are identical, as well as the equalizing marginals condition. Rewriting the equations gives both conditions in the statement. It remains to verify that there exists $\mu^S, \mu^F > 0$ that satisfy both conditions. In fact, we have
$$1/\mu^F=\gamma\cdot \left(\frac{L}{H}+\frac{2v'(1/2)}{v^2(1/2)}\cdot L\right) + (1-\gamma) > 0$$
and $\mu^S = (1+\frac{2v'(1/2)}{v^2(1/2)}\cdot H)\cdot \mu^F > 0$.
The lemma then follows from \Cref{theo:spa_fpa__subgame}.
\end{proof}

 The revenue of platform 1 (SPA) is $\int_{0}^{1/2} \gamma \mu^Sv_1(q)dq+\int_{1/2}^1\gamma \mu^S v_2(q)dq=2\mu^S\gamma L$. The revenue of platform 2 (FPA) is $\int_{0}^{1/2} (1-\gamma) \mu^Fv_2(q)dq+\int_{1/2}^1(1-\gamma) \mu^F v_1(q)dq=2\mu^S\gamma L=2\mu^F(1-\gamma) H$.  By \Cref{lem:sym:spfp} the total revenue of both platforms is $2H$.

\paragraph{Case 4: (SPA, FPA)} This case is analogous to the previous case by swapping the market share parameter. We have the following lemma analogous to \Cref{lem:sym:spfp}. The proof is omitted.
\begin{lemma}\label{lem:sym:fpsp}
There exists a symmetric equilibrium for the advertisers in the (FPA, SPA) profile such that $\mu_1^S=\mu_2^S=\tilde{\mu}^S, \mu_1^F=\mu_2^F=\tilde{\mu}^F$ where
\begin{itemize}
    \item $\frac{\tilde{\mu}^S}{\tilde{\mu}^F}=1+\frac{2v'(1/2)}{v^2(1/2)}\cdot H,$
    \item $\tilde{\mu}^S (1-\gamma) L+\tilde{\mu}^F \gamma H = H$.
\end{itemize}
\end{lemma}

Finally, we can write the payoffs for each platform under all possible action profiles. In particular, note that the welfare of every action profile is $2H$. So long as the payoff matrix is not degenerate, the Nash equilibria of this game will be exactly one of (SPA, SPA) or (FPA, FPA). Surprisingly, which of these two profiles is the Nash equilibrium will depend only on the shape of the valuation and not on the market share $\gamma$. 

  \begin{table}[h!]
  \centering
    \setlength{\extrarowheight}{8pt}
    \begin{tabular}{cc|c|c|}
      & \multicolumn{1}{c}{} & \multicolumn{2}{c}{Ch 2}\\
      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{SPA}  & \multicolumn{1}{c}{FPA} \\\cline{3-4}
      \multirow{2}*{Ch 1}  & SPA & $(2\gamma H, 2(1-\gamma) H)$ & $(2\mu^S\gamma L, 2\mu^F(1-\gamma)H)$ \\\cline{3-4}
      & FPA & $(2\tilde{\mu}^F\gamma H, 2\tilde{\mu}^S(1-\gamma) L)$ & $(2\gamma H, 2(1-\gamma) H)$ \\\cline{3-4}
    \end{tabular}
  \end{table}
  

\begin{theorem}\label{lem:symeq}
Let $Q=\frac{L}{H}+\frac{2v'(1/2)}{v^2(1/2)}\cdot L$ be the parameter that only depends on $v(\cdot)$ (independent of the market share $\gamma$). If $Q>1$, then (SPA, SPA) is the only NE of the game. If $Q<1$, then (FPA, FPA) is the only NE. If $Q=1$, then all four profiles of the game have the same outcome.  
%$$\frac{L}{H}+\frac{2v'(1/2)}{v^2(1/2)}\cdot L>\max\left\{\frac{\gamma}{1-\gamma}, \frac{1-\gamma}{\gamma}\right\}$$
%(FPA, FPA) is the only pure NE if
%$$\frac{L}{H}+\frac{2v'(1/2)}{v^2(1/2)}\cdot L<\min\left\{\frac{\gamma}{1-\gamma}, \frac{1-\gamma}{\gamma}\right\}$$
%Otherwise, there is no pure NE in the game.
\end{theorem}

Before going to the proof, we notice that
$$\compet=1-\frac{\int_0^1 |v_1(q)-v_2(q)|dq}{\int_0^1 \max\{v_1(q), v_2(q)\}dq}=1-\frac{2(H-L)}{2H}=\frac{L}{H}$$
$$\ela(1/2) = 1+\frac{2v'(1/2)}{v^2(1/2)}\cdot H. $$

Thus $Q=\ela(1/2)\cdot \compet$. So \Cref{lem:symeq} is a restatement of \Cref{thm:symeq} and \Cref{thm:market_share_sym} when there are 2 platforms.

\begin{proof}[Proof of \Cref{lem:symeq}]

Let $a=2\gamma H, b=2\tilde{\mu}^F\gamma H, c=2\mu^S\gamma L$, the game can be rewritten as the following table:

  \begin{table}[H]
  \centering
    \setlength{\extrarowheight}{8pt}
    \begin{tabular}{cc|c|c|}
      & \multicolumn{1}{c}{} & \multicolumn{2}{c}{Ch 2}\\
      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{SPA}  & \multicolumn{1}{c}{FPA} \\\cline{3-4}
      \multirow{2}*{Ch 1}  & SPA & $(a, 2H-a)$ & $(c, 2H-c)$ \\\cline{3-4}
      & FPA & $(b, 2H-b)$ & $(a, 2H-a)$ \\\cline{3-4}
    \end{tabular}
  \end{table}

{Observe that in order for (SPA, SPA) to be a Nash equilibrium we need that $a > b$, $2H-a > 2H-c$ (or $c > a$). Analogously, in order for (FPA, FPA) to be a Nash equilibrium we need that $c < a$ and $2H- a > 2H - b$ (or $a < b$). We will now show that $Q < 1 \iff b > a \iff a > c$.}
%Observe that in order for (SPA, SPA) to be a Nash equilibrium we need that $a > c$, $2H-a > 2H-b$ (or $b > a$). Analogously, in order for (FPA, FPA) to be a Nash equilibrium we need that $c > a$ and $2H- a > 2H - b$ (or $a > b$). We will now show that $b > a > c \iff Q < 1$. 

\begin{claim}
{$Q < 1 \iff b > a \iff a > c$.}
%$$b > a > c \iff Q < 1$$.
\end{claim}

\begin{proof}
By \Cref{lem:sym:fpsp},
\begin{align*}
(1-\gamma) H Q \tilde{\mu}^F +\tilde{\mu}^F\gamma H & = H \\
1/\tilde{\mu}^F & =Q (1-\gamma)+\gamma.
\end{align*}
Similarly by \Cref{lem:sym:spfp}, 
%$$\mu^S\gamma L+\frac{\mu^S(1-\gamma) H}{1+\frac{2v'(1/2)}{v^2(1/2)}\cdot H}=H$$

\begin{equation}\label{equ:mirror_mu_F}
1/\mu^F=Q \gamma+(1-\gamma)
\end{equation}

By definition,
\begin{align*}
a<b & \iff \tilde{\mu}^F>1 \\ 
& \iff (\frac{L}{H}+\frac{2v'(1/2)}{v^2(1/2)}\cdot L)(1-\gamma)+\gamma<1 \\ 
& \iff Q < 1 \\ 
a>c & \iff \mu^S < H/L \\ 
& \iff 1/\mu^F > \frac{L}{H}+\frac{2v'(1/2)}{v^2(1/2)}\cdot L \\
& \iff Q < 1.
\end{align*}
Thus if $Q < 1$ we have that $b>a>c$ and if $Q > 1$ we have that $c>a>b$. 
\end{proof}

Therefore, if $Q > 1$, the only equilibrium is (SPA, SPA). If $Q < 1$, the only equilibrium is (FPA, FPA). If $Q = 1$, then the game is degenerate and all action profiles have the same payoffs. 
\end{proof}

\subsection{Equilibrium for Standard Valuations}\label{subsec:mirror_case_study}

We apply the result of \Cref{lem:symeq} to show that (SPA, SPA) is the only Nash equilibrium for many standard valuations.

\subsubsection{Polynomial valuations $v(q)= \sum_{i \geq 1} \alpha_i q^{i} (\alpha_i\geq 0)$}

%\arielnote{Do we care about these subcases at this point? We still needed to confirm that landscapes were concave. }

%We can specialize the results from the previous section to the case of polynomial valuations. 

\begin{corollary}
For polynomial valuations with positive coefficients and no constant term, (SPA, SPA) is always the only Nash equilibrium. 
\end{corollary}

\begin{proof}
Let $v(q) = \sum_{i \geq 1} \alpha_i q^i$.

\begin{align*}
    v'(1/2) &= \sum_i \alpha_i \cdot i \cdot 2^{1-i} \\ 
    v^2(1/2) &= \left(\sum_i \alpha_i 2^{-i}\right)^2 \\  
    L &= \int_{0}^{1/2} \sum_i \alpha_i q^i dq = \sum_i \frac{\alpha_i 2^{-(i+1)}}{(i+1)}
\end{align*}

First note that if $L = 0$, then all $\alpha_i$ must be $0$, in which case $H$ is also $0$ and the game is degenerate, hence any action profile would be a Nash equilibrium. Assume $L > 0$ for the rest of this proof. We will prove that $Q > 1$ directly by showing that $2 \cdot \frac{2v'(1/2)}{v^2(1/2)} \cdot L \geq 1$. By Cauchy-Schwarz we know that 

\begin{align*}
    v'(1/2) \cdot L \geq \left(\sum_i \frac{\alpha_i 2^{-i} \sqrt{i}}{\sqrt{i+1}} \right)^2. \\ 
\end{align*}

Multiplying both sides by 2 and observing that $2\frac{i}{i+1} \geq 1$ (for all $i \geq 1$) gives the inequality. Since $L > 0$, then $Q>1$. 
\end{proof}

\begin{corollary}
The above proof can be extended to polynomials with constant terms $a_0$ so long as $a_0 \geq 2v(1/2) - 2v'(1/2) - 1$. 
\end{corollary}

\begin{comment} --- 
We can specialize the results from the previous section to the case of monomial valuations $v(q) = q^{\alpha}$ for some $\alpha > 0$.

\begin{corollary}
For monomial valuations, (SPA, SPA) is always the only Nash equilibrium. 
\end{corollary}

\begin{proof}

Because of Lemma~\ref{lem:symeq}, all we need to do is compute $Q$. 

\begin{align*}
H & =\int_{1/2}^{1}q^{\alpha}dq = \frac{1}{\alpha+1}(1-2^{-(\alpha+1)}) \\ 
L & =\int_{0}^{1/2}q^{\alpha}dq = \frac{1}{\alpha+1}\cdot 2^{-(\alpha+1)}
\end{align*}

Therefore, we have that 

\begin{align*}
Q = \frac{L}{H}+\frac{2v'(1/2)}{v^2(1/2)}\cdot L & = \frac{2^{-(\alpha+1)}}{(1-2^{-(\alpha+1)}}+\frac{2\cdot \alpha 2^{1-\alpha}}{2^{-2\alpha}}\cdot \frac{1}{\alpha+1}\cdot 2^{-(\alpha+1)} \\ & =\frac{2\alpha}{\alpha+1}+\frac{1}{2^{\alpha+1}-1} \\ 
\end{align*}

The function $f(\alpha)=\frac{2\alpha}{\alpha+1}+\frac{1}{2^{\alpha+1}-1}$ is a strictly increasing function in $[0,\infty)$ with $f(0)=1$. Thus $f(\alpha) > 1$ for all $\alpha>0$. Thus (SPA, SPA) is the only NE. 

\end{proof}

\end{comment}

\subsubsection{Fixed crossing point}

Given Lemma~\ref{lem:symeq}, we can think of how the equilibrium changes for families of valuations with, say, fixed crossing points. For this section, assume $v(1/2) = 1/2$. 

\begin{corollary}
For linear valuations with $v(1/2) = 1/2$, (SPA, SPA) is the unique Nash equilibrium. 
\end{corollary}

\begin{proof}
We will again show directly that $Q \geq 1$. We consider two sub-cases. Let $v(q) = \alpha q + \beta$ be the valuation, and since $v(1/2)=1/2$ we know that $\beta = 1/2 - \alpha/2$. Also, note that $L + H = 1/2$. 

\textbf{Subcase 1: $0 < \alpha < 1$.} In this case we can compute $L$ directly. 

\begin{align*}
    L &= \int_{0}^{1/2} (\alpha q + 1/2 - \alpha/2) dq \\ 
    & = \alpha/8 + 1/4- \alpha/4 =  1/4-\alpha/8.\\  
\end{align*}

Thus, $Q = \frac{1/4 - \alpha/8}{1/4+\alpha/8}+2\frac{\alpha}{1/4}(1/4-\alpha/8) = \frac{2-\alpha}{2+\alpha} + \alpha \cdot (2-\alpha)$. It is easy to verify that for $0 \leq \alpha \leq 1$, $Q \geq 1$ with equality only when $\alpha = 0$.

\textbf{Subcase 2: $\alpha > 1$.} In this case, the function has a $y$-intercept below $0$. Instead of assuming that the valuations are negative, we will truncate the valuation to $v^{+}(q) = \max\{v(q),0\}$. The valuation becomes non-negative starting at $q = 1/2-\frac{1}{2\alpha}$. Here we have $L = \frac{\frac{1}{2\alpha} \frac{1}{2}}{2}=\frac{1}{8\alpha}$. Therefore, $Q = \frac{\frac{1}{8\alpha}}{1/2-\frac{1}{8\alpha}}+2\frac{\alpha}{1/4}\frac{1}{8\alpha} =\frac{1}{4\alpha-1}+1$. Since $Q \geq 1$, we get that in this case too (SPA, SPA) is the unique NE. 

\end{proof}
    
\subsubsection{Fixed slope} 

Similar to the previous case, we can consider what happens when we consider linear functions with $v'(1/2) = \alpha$ for some fixed $\alpha$. Without loss of generality, assume $\alpha = 1$. Let $v(q) = q + \beta$. 

\begin{corollary}
For linear functions with $v'(1/2) = 1$, the unique equilibrium will be (SPA, SPA). 
\end{corollary}

\begin{proof}
Then $L = \frac{2\beta + 1/2}{4}$, $H = \frac{2\beta+3/2}{4}$. Therefore, $Q = \frac{2\beta+1/2}{2\beta+3/2}+2\frac{2\beta+1/2}{(\beta+1/2)^2}$. It is easy to verify that for $\beta > 0$, $Q > 1$. Note that we need $\beta > -1/2$ since otherwise $v(1/2) < 0$ in which case the analysis would not hold. For $0 > \beta > -1$, we again truncate the negative part of the valuation to $0$. We can recompute $L, H$ in this case. We get that $L = \frac{(1/2+\beta)v(1/2)}{2}, H = -\beta + \frac{(1/2+\beta)(v(1/2)+1)}{2}$. Ultimately we get that $Q = \frac{(1/2+\beta)v(1/2)}{-2\beta+(1/2+\beta)(v(1/2)+1)}+2\frac{1}{v^2(1/2)}\frac{(1/2+\beta)v(1/2)}{2}$. Note that $1/2+\beta = v(1/2)$. Therefore, the second term alone is already $1$. Since the first term is non-negative, we get that $Q \geq 1$, and assuming $L > 0$, $Q > 1$. 

\end{proof}



\subsubsection{Exponential valuations}

\begin{corollary}
For exponential valuations $v(q) = e^{\alpha q}-1$ with $\alpha > 0$, it is always a NE to have (SPA, SPA). 
\end{corollary}

\begin{proof}
We will prove that the second term of $Q$ is already greater than $1$ for all $\alpha > 0$.

\begin{align*}
    L & = \int_0^{1/2} (e^{\alpha x} - 1) dx \\
    & = \frac{e^{\alpha/2}}{\alpha}-1/2. 
\end{align*}

Furthermore, $v'(1/2) = \alpha (e^{\alpha/2})$, $v^2(1/2) = (e^{\alpha/2}-1)^2$. Then the condition becomes 

\begin{align*}
    \frac{e^{\alpha/2}(2e^{\alpha/2}-\alpha)}{(e^{\alpha/2}-1)^2}.
\end{align*}

It is easy to verify that this expression is at greater than 1 for $\alpha > 0$. 

\end{proof}

\subsection{Multiple Platforms} \label{subsec:mirror_multi_platforms}

In this section we prove \Cref{thm:market_share_sym} using the results we developed in \Cref{subsec:mirror_two_platform}.

\begin{proof}[Proof of \Cref{thm:market_share_sym}]
Fix any platform $j$ and the auction choices of the other platforms. We are going to analyze platform $j$'s best response at the current outcome. Let $\gamma'$ be the total market share of all other platforms that choose SPA. Then the total market share of all other platforms that choose FPA is $1-\gamma'-\gamma_j$. We compute as follows the advertiser equilibrium and revenue of platform $j$ if the platform chooses SPA and FPA respectively.

To achieve this, consider any auction outcome and denote $\gamma\in [0,1]$ the total market share of the platforms that choose SPA. By symmetry, advertisers will use the same multiplier on all platforms that chooses SPA, which we denote as $\mu^S(\gamma)$. Similarly denote $\mu^F(\gamma)$ the multipliers on the FPA platforms. We notice that by merging all SPA platforms and FPA platforms respectively, the advertiser equilibrium is equivalent to the one of the (SPA, FPA) profile in the two-platform setting. By \Cref{lem:sym:spfp}, $(\mu^S(\gamma), \mu^F(\gamma))$ satisfy that 
\begin{itemize}
    \item $\frac{\mu^S(\gamma)}{\mu^F(\gamma)}=1+\frac{2v'(1/2)}{v^2(1/2)}\cdot H,$
    \item $\mu^S(\gamma)\cdot \gamma L+\mu^F(\gamma)\cdot (1-\gamma) H = H.$
\end{itemize}
Or equivalently (by \Cref{equ:mirror_mu_F}), 
$$\mu^F(\gamma) = \frac{1}{Q\gamma+1-\gamma},\qquad \mu^S(\gamma)=\mu^F(\gamma)\cdot \left(1+\frac{2v'(1/2)}{v^2(1/2)}\cdot H\right)=\mu^F(\gamma)\cdot Q\cdot \frac{H}{L}$$

\paragraph{The platform chooses SPA} We notice that SPA has a total market share of $\gamma'+\gamma_j$. Thus both advertisers use multiplier $\mu^S(\gamma'+\gamma_j)$ for platform $j$. Recall that in the symmetric equilibrium, advertiser $1$ wins query $q\in[0,1/2]$ and advertiser $2$ wins query $q\in(1/2,1]$. The revenue of platform $j$ is 
$$\mathcal{R}_S=\gamma_j\cdot \int_0^{\frac{1}{2}}\mu^S(\gamma'+\gamma_j)\cdot v_1(q)dq+\gamma_j\cdot \int_{\frac{1}{2}}^1\mu^S(\gamma'+\gamma_j)\cdot v_2(q)dq=2\gamma_j\cdot \mu^S(\gamma'+\gamma_j)\cdot L.$$

\paragraph{The platform chooses FPA} Now SPA has a total market share of $\gamma'$. Thus both advertisers use multiplier $\mu^F(\gamma')$ for platform $j$. The revenue of platform $j$ is 
$$\mathcal{R}_F=\gamma_j\cdot \int_0^{\frac{1}{2}}\mu^F(\gamma')\cdot v_2(q)dq+\gamma_j\cdot \int_{\frac{1}{2}}^1\mu^F(\gamma')\cdot v_1(q)dq=2\gamma_j\cdot \mu^F(\gamma')\cdot H.$$

We now compare the revenue of both choices:
\begin{align*}
\frac{\mathcal{R}_S}{\mathcal{R}_F}&=\frac{\mu^S(\gamma'+\gamma_j)}{\mu^F(\gamma')}\cdot \frac{L}{H}=Q\cdot \frac{\mu^F(\gamma'+\gamma_j)}{\mu^F(\gamma')}=Q\cdot \frac{Q\gamma'+1-\gamma'}{Q(\gamma'+\gamma_j)+1-\gamma'-\gamma_j}\\
&=Q\cdot \left(1-\frac{(Q-1)\cdot \gamma_j}{Q(\gamma'+\gamma_j)+1-\gamma'-\gamma_j}\right)
\end{align*}
Thus
$$\mathcal{R}_S>\mathcal{R}_F\Leftrightarrow \frac{(Q-1)\cdot \gamma_j}{Q(\gamma'+\gamma_j)+1-\gamma'-\gamma_j}<\frac{Q-1}{Q}\Leftrightarrow (Q-1)\cdot (1-\gamma_j+(Q-1)\gamma') > 0$$

We notice that $1-\gamma_j+(Q-1)\gamma'>1-\gamma_j-\gamma'\geq 0$ since $Q>0$ and $\gamma'+\gamma_j\leq \sum_k \gamma_k=1$. Thus $\mathcal{R}_S>\mathcal{R}_F\Leftrightarrow Q>1$. This finishes the proof: If $Q>1$, then SPA dominates FPA for any platform $j$ and any auction profile of the other platforms. Thus there is a unique platform equilibrium where every platform chooses SPA. On the other hand, if $Q<1$, then FPA is a dominate strategy for any platform. Thus the unique Nash equilibrium of the game is all platforms choosing FPA.
\end{proof}

\section{Missing Proofs from Section~\ref{sec:linearvsconstant}}


For this case, we can compute optimal bids for each of the strategy pairs the platforms might employ. This in turn allows us to determine the Nash equilibria of the platform-advertiser game as a function of $\alpha$. Before we can state the main result of this section, we will restrict our attention to a range of $\alpha$. As it will turn out, $\alpha$ not in this range are easy to solve and strategically not as compelling. 

\begin{proof}[Proof of Claim~\ref{cl:alpharange}]
For values of $\alpha \not \in [2,4]$, we claim that the (SP, SP) subgame will have an equilibrium where a single advertiser wins all or virtually all queries. Because of this effective lack of advertiser competition, we will rule out these values of $\alpha$. 

Regardless of $\alpha$, it will turn out that a dominant strategy for the second advertiser is to set a bid multiplier of $\mu_2 = 2$. This is because for any queries they win they will be paying $\int_0^{q_S} \mu_1 q dq$, where $q_S$ satisfies $\mu_1 q_S = 2$. Therefore, they will at most $\mu_1 q_S^2/2 \leq q_S$, which is the total value for the queries they would win. Setting a multiplier lower than $2$ is weakly dominated by setting a multiplier of $2$ since they win weakly more queries while not violating their target constraint. Setting a multiplier higher than $2$ is dominated since they will be violating their target constraint. 

First we consider the case where $\alpha < 2$. Since $\mu_2 = 2$, then the price on any impressions the first advertiser wins will be $2 > \alpha$. Therefore, winning any queries will cause the first advertiser to violate their target constraint. Because of this, the first advertiser will set $\mu_1 < 2$. Whatever $\mu_1$ is, the second advertiser will win all queries and still satisfy their target constraint. 

Next we consider the case where $\alpha > 4$. Since $\mu_2 = 2$, again the first advertiser faces a price of $2$ on any queries they win. Their total payment is $2 (1-q_S)$, and their total value for these queries is $\alpha/2 (1-q_S^2)$. If $\alpha \geq 4$, then the value will always exceed the cost. Therefore, they are willing to set a bid multiplier of $\mu_1 = \infty$, which would cause them to win virtually all queries. Another way to phrase this last result is that for any $\mu_1 = M >> 2$, setting a multiplier of $M' > M$ is a better strategy since it will win more queries while satisfying the target constraint.    
\end{proof}



%\mingfeinote{TODO: State the theorem as the transition with 4 ranges.}


The proof of Theorem~\ref{thm:mainconstantvslinear} relies on the analysis of the three different subgames -- (FPA, FPA), (SPA, SPA) and (FPA, SPA). We first compute the equilibrium bid multipliers for each subgame. These in turn define the revenue (as a function of $\alpha$) that each of the platform gets. Once we have all payoffs, we can derive conditions under which the action profiles are equilibria. As it turns out, there exist values of $\alpha$ that support all possible pure Nash equilibria in this game. 

The first subgame where both platforms use FPA is easy to analyze: advertisers will use bid multipliers of $1$, platforms will allocate efficiently and achieve a combined revenue equal to the liquid welfare.

\begin{claim}\label{cl:FPAlinear}
In the (FPA, FPA) subgame, the advertisers will bid truthfully and the allocation will be efficient. The revenue of each platform in this case is $(\alpha+\frac{1}{\alpha})/2$. 
\end{claim}

\begin{proof}
 Because platforms are identical and advertisers are being first-priced, then each advertiser uses a bid multiplier $\mu_i^F=1$ in equilibrium. To see this, fix $\mu_1^F=1$ and consider possible responses by the second advertiser. Using a bid multiplier $\mu_2^F>1$ will result in an allocation where aggregate spend is greater than aggregate value. Using a bid multiplier $\mu_2^F < 1$ is dominated since the advertiser can raise their bid to $1$ and win weakly more queries while ensuring that their aggregate spend is not greater than their aggregate value. Even though the bidders are not identical in this case, the same reasoning holds if we fix $\mu_2^F = 1$ and compute a best, undominated response for advertiser $1$. 
Thus, each platform extracts the full liquid welfare from the advertisers. Finally, observe that $q^1_F = q^2_F = \frac {1}{\alpha}.$ The revenue the each platform gets is given by  $$1 + \frac{1}{2} (\alpha-1)(1-q^1_{F}) = \frac{\alpha^2+1}{2\alpha}.$$
\end{proof}

The inefficiencies (and intricacies) of this family of valuations begin with the subgame where both platforms use SPA. In this case we first show that advertiser 2 will always bid with a multiplier of $2$. This, combined with other optimality conditions, allows us to pin down the optimal multiplier for advertiser 1, as  well as the overall revenue of the platforms as a function of $\alpha$. 

\begin{claim}\label{cl:SPAlinear}
In the (SPA, SPA) subgame, advertiser 2 will use a bid multiplier of $\mu_2 = 2$, advertiser 1 will use a bid multiplier of $4/\alpha - 1$. The revenue of each platform in this case is $3-\frac{4}{\alpha}$. 
\end{claim}



\begin{proof}
Since the platforms are indistinguishable, we will solve for a symmetric equilibrium where advertisers use the same multipliers for both platforms, and both platforms get the same revenue. The bid multipliers $\mu_i^S$ are chosen so that both advertisers meet their target constraint. There are three equations that govern the unknowns in this setting. 

\begin{align*}
    \mu_2^S & = \mu_1^S \alpha q_S, \\
    \mu_2^2(1-q_S) & = \int_{q_S}^{1} \alpha q dq = \alpha \frac{(1-q_S^2)}{2}, \\ 
    q_S &= \int_{0}^{q_S} \mu_1^S \alpha q dq = \mu_1^S \alpha \frac{q_S^2}{2}.\\  
\end{align*}

The first equation establishes that $q_S$ is the point at which the first advertiser becomes the highest bidder for the first time. The second equation ensures that the spend by the first advertiser (which depends on the second advertiser's multiplier) equals their value for the acquired queries. The last equation does the same for the second advertiser (whose spend depends on the first advertiser's multiplier). From the first and last equation we can infer directly that $\mu_2^S = 2$. This in turn implies that $q_S = \frac{4}{\alpha}-1$ and $\mu_1^S = \frac{2}{4-\alpha}$. The revenue each platform gets is 
%$$q_S + \alpha/2 (1-q_S^2)= \frac 4 \alpha + \alpha -3.$$
$$q_s+2(1-q_s) = 3 - \frac{4}{\alpha}.$$



%By the same logic as before, $\mu_2^S = 2$. Hence, the problem is to find $q_S$ so that Bidder $1$ meets its target.

\end{proof}


Finally, the most intricate case is that where one platform uses SPA and the other uses FPA. Because the platforms are no longer symmetric, each advertiser may use a different multiplier on each platform. Interestingly, the multipliers for advertiser 2 are easy to obtain and understand: the advertiser will still use a multiplier of $2$ on the SPA platform and a multiplier of $1$ on the FPA platform. Utilizing the results from the previous sections, we are able to mathematically solve for the remaining variables in this scenario as a function of $\alpha$. However, those solutions are not as elegant to present. 

\begin{claim}\label{cl:FPASPAlinear}
In the (FPA, SPA) subgame, advertiser 2 will use a bid multiplier of $\mu_2^S = 2$ on the SPA platform and a multiplier of $\mu_2^F = 1$ on the FPA platform. The multipliers of advertiser 1 depend on $\alpha$ and $q_F$, the query where advertiser 1 starts winning queries on the FPA platform. The revenues of each platform can be computed as a function of $\alpha, q_F$ (where $q_F$ is uniquely determined by $\alpha$). 
\end{claim}


\begin{proof}

There are six variables to solve for $\mu_1^F, \mu_1^S, \mu_2^F, \mu_2^S, q_F, q_S$. We first write the equations which establish that $q_F, q_S$ are the points at which the second advertiser starts losing queries and the first advertiser starts winning them.

\begin{align}
    \mu_2^F & = \mu_1^F \alpha q_F \label{eq:FPSPqF} \\ 
    \mu_2^S & = \mu_1^S \alpha q_S \label{eq:FPSPqS} 
\end{align}

The remaining equations come from the analysis on the previous section. We just instantiate Eqs.\eqref{eq:intrabidder1}-\eqref{eq:tcpa-final-spa-fpa} for the valuations $v_1(q)=\alpha q$, $v_2(q)=1$. 

\begin{align}
    \frac{\mu_1^S}{\mu_1^F} & =  \frac{(1+q_F^2)}{2q_F^2} \label{eq:linearintrabidder}\\ 
    \frac{\mu_2^S}{\mu_2^F} & = 2 \label{eq:constantintrabidder} \\ 
    (\mu_1^F-1)\frac{(1-q_F^2)\alpha}{2} &= \frac{(1-q_S^2)\alpha}{2} - \mu_2^S(1-q_S) \label{eq:lineartarget} \\
    (\mu_2^F-1)q_F &= q_S - \alpha \frac{q_S^2 \mu_1^S}{2} \label{eq:constanttarget}  
\end{align}

Substituting Eqs.~\ref{eq:FPSPqS},~\ref{eq:constantintrabidder} into Eq.~\ref{eq:constanttarget}, we get that 

\begin{align*}
    (\mu_2^F-1) q_F = q_S - \mu_2^F q_S = q_S (1-\mu_2^F). 
\end{align*}

Because $q_S, q_F \geq 0$, the expression above can only hold if $\mu_2^F = 1$. Therefore, by Eq.~\ref{eq:constantintrabidder}, $\mu_2^S = 2$. We write the remaining variables in terms of $q_F$: 

\begin{align*}
    \mu_1^F &= \frac{1}{\alpha q_F} \\ 
    \mu_1^S &= \frac{(1+q_F^2)}{2\alpha q_F^3} \\ 
    q_S &= \frac{4q_F^3}{(1+q_F^2)}
\end{align*}
    
Finally, we can substitute all of these and write Eq.~\ref{eq:lineartarget} fully as a function of $q_F$ (and $\alpha$). 

\begin{align*}
    \left(\frac{(1-\alpha q_F)}{\alpha q_F}\frac{(1-q_F^2) \alpha}{2} \right) & = \left(1-\frac{(4q_F^3)^2}{(1+q_F^2)^2}\right) \frac{\alpha}{2} - 2\left(1-\frac{4q_F^3}{(1+q_F^2)}\right). 
\end{align*}

Rewriting $q_F =x$,  


$$ 17 \alpha x^7 - 17 x^6 + 4x^5 - 17x^4 + (8-3 \alpha) x^3 + x^2 + (4-2 \alpha)x + 1 = 0. $$

Finally, we can write $\alpha$ as a function of $x$. 

\begin{align*}
    \alpha = \frac{17x^6-4x^5+17x^4-8x^3-x^2-4x-1}{17x^7-3x^3-2x}.
\end{align*}

With this expression relating $\alpha$ and $q_F$ we can empirically plot their relationship and observe that $q_F$ is monotone decreasing in $\alpha$. This in particular implies that as $\alpha$ increases, advertiser $1$ wins more queries in the FPA platform. 


\begin{claim}\label{cl:alphamonotone}
For the (FPA, SPA) subgame, $q_F$, the point at which advertiser $1$ starts winning queries in the FPA platform, is strictly decreasing in $\alpha$. 
\end{claim}

We can now compute the revenue each platform gets. The platform running First Price gets revenue 

\begin{align*}
    \mu_2^F q_F + \int_{q_F}^{1} \mu_1^F \alpha q dq & = q_F + \frac{\alpha (1-q_F^2)}{2 \alpha q_F} \\ 
    & = \frac{1+q_F^2}{2q_F}. 
\end{align*}

The platform running Second Price gets revenue 

\begin{align*}
    \int_0^{q_S} \mu_1^S \alpha q dq + \int_{q_S}^{1} \mu_2^S dq & = \frac{1+q_F^2}{4q_F^3} \cdot  \left(\frac{4q_F^3}{(1+q_F^2)}\right)^2 + 2(1-q_S) \\
    & = \frac{4q_F^3}{(1+q_F^2)}+2\left(1-\frac{4q_F^3}{1+q_F^2}\right) = 2-\frac{4q_F^3}{1+q_F^2}. 
\end{align*}
\end{proof}



Once we have Claims~\ref{cl:FPAlinear},~\ref{cl:SPAlinear},~\ref{cl:FPASPAlinear} we can write the payoff matrix for each platform under all action profiles. With this symmetric matrix in hand, we can exactly determine the conditions (and values of $\alpha$) under which each action profile is a possible equilibrium of the game. We can now write the full payoff matrix for the ensuing game between the platforms. We are now ready to present the main result of this section, the proof of Theorem~\ref{thm:mainconstantvslinear}. 



%Where $q_S= 2 q_F^3$ and $q_F$ solves the equation$$ 1/2 (1-q_F^2)/q_F + \alpha/2 (q_S^2 - q_F^2) = -2(1-q_S).$$


  \begin{table}[h!]
  \centering
    \setlength{\extrarowheight}{8pt}
    \begin{tabular}{cc|c|c|}
      & \multicolumn{1}{c}{} & \multicolumn{2}{c}{Platform 2}\\
      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{SPA}  & \multicolumn{1}{c}{FPA} \\\cline{3-4}
      \multirow{2}*{Platform 1}  & SPA & $(3-4/\alpha, 3-4/\alpha)$ & $(2- q_S,\frac {1+q_F^2}{2q_F})$ \\\cline{3-4}
      & FPA & $(\frac {1+q_F^2}{2q_F},2- q_S)$ & $(\frac{\alpha^2+1}{2\alpha},\frac{\alpha^2+1}{2\alpha})$ \\\cline{3-4}
    \end{tabular}
        \caption{Payoff matrix for the platforms' game after solving for the advertisers' subgame equlibrium, for the valuatiosn described in Section~\ref{sec:linearvsconstant}}
    \label{table:lingame}
  \end{table}
 
\begin{proof}[Proof of Theorem~\ref{thm:mainconstantvslinear}.]

Before considering the conditions under which each profile is an equilibrium, let us review the conditions that all candidates must satisfy in order to be feasible solutions to our problem. 

\begin{align*}
    q_F & \in [0,1] \\ 
   2 &\leq \alpha \leq 4 \\
    \alpha &= \frac{17{q_F}^6-4q_F^5+17q_F^4-8q_F^3-q_F^2-4q_F-1}{17q_F^7-3q_F^3-2q_F} \in [2,4] \\ 
    & \rightarrow x_1 = .237818 \leq q_F \leq x_5 = .610502, 
\end{align*}

Let us rewrite the payoff matrix as follows. Let $x=3-4/\alpha$, $y = 2-q_S$, $z=\frac{1+q_F^2}{2q_F}$, $w=\frac{\alpha^2+1}{2\alpha}$. In these terms, (SPA, SPA) is a pure NE when $x > z$, (FPA, FPA) is a pure NE when $w > y$. Both of these conditions can happen simultaneously for a small range of values of $\alpha$, and in that case their mixture is also a Nash equilibrium of the game. If neither of these conditions holds, then (FPA, SPA), (SPA, FPA) and a mixture between these two are the only Nash equilibrium.

\begin{itemize} 
\item If $x > z \rightarrow x_2 \leq q_F \leq x_4$, where $x_2 = .287407, x_4 = .565389$. 
\item If $w > y \rightarrow x_1 \leq q_F \leq x_3$, where $x_1 = .237818, x_3 = .295027$.
\item If both $x > z \land w > y \rightarrow x_2 \leq  q_F \leq x_3$.   
\item If $z > x \land y > w \rightarrow q_F \geq x_4 \lor q_F \leq x_1$. 
\end{itemize}

Therefore, if 
\begin{itemize} 
\item $x_1 \leq q_F \leq x_2$, (FPA, FPA) is the unique Nash equilibrium, 
\item $x_2 \leq q_F \leq x_3$, then (SPA, SPA), (FPA, FPA) and a mixture between the two are all Nash equilibria, 
\item $x_3 \leq q_F \leq x_4$, (SPA, SPA) is the unique Nash equilibrium,
\item $x_4 \leq q_F \leq x_5$, then (FPA, SPA), (SPA, FPA) and a mixture of the two are all equilibria. 
\end{itemize}

Finally, because for $\alpha \in [2, 4]$, $q_F$ is monotone decreasing in $\alpha$, we get that there exist $\alpha_0 = 2 < \alpha_1 < \alpha_2 < \alpha_3 < \alpha_4 =4$ where the equilibria change as indicated above.

Therefore, if 
\begin{itemize} 
\item $4 \geq \alpha \geq \alpha_3 = 3.5822$, (FPA, FPA) is the unique Nash equilibrium, 
\item $\alpha_3 \geq \alpha \geq \alpha_2 = 3.52753$, then (SPA, SPA), (FPA, FPA) and a mixture between the two are all Nash equilibria, 
\item $\alpha_2 = 3.52753 \geq \alpha \geq \alpha_1 = 2.1822$, (SPA, SPA) is the unique Nash equilibrium,
\item $\alpha_1 = 2.1822 \geq \alpha \geq \alpha_0 = 2$, then (FPA, SPA), (SPA, FPA) and a mixture of the two are all equilibria. 
\end{itemize}

\end{proof}



\section{Missing Proofs From Section ~\ref{sec:expvsexp}}

%This case should provide sharp contrast with both cases in Section~\ref{sec:inefficiency_free},~\ref{sec:efficiencybidding} for the following reasons.

%Firstly, because both valuations have exponential shapes the elasticity of the valuations will be constant. Secondly, the valuations themselves will be pretty close to each other, which implies that the allocations will be close to fully-efficient. This sits between the two previous examples where the allocation was always efficient (Section~\ref{sec:inefficiency_free}) and the allocation was somewhat inefficient~\ref{sec:efficiencybidding} for some values of $\alpha$. Therefore, this example will have valuations with constant elasticity (as a function of the parameter $\alpha$) and relatively low competition (as a function of $\alpha$) (or relatively high efficiency). In this case, because $1/4 \leq \alpha \leq 1/2$, the second advertiser will have a higher valuation for earlier queries but will eventually fall below the valuation of the first advertiser. The main result of this section is that for $1/4 \leq \alpha \leq 1/2$, SP is a dominant strategy of this game. 

Just like the proof of Theorem~\ref{thm:mainconstantvslinear}, the proof of Theorem~\ref{thm:expequilibria} will begin by finding the subgame equilibria for each of the three possible subgames. We will also compute each platforms' payoffs under the advertisers' equilibrium multipliers. Finally, we will compute the payoff matrix and prove numerically that SP is a dominant strategy of the game. 

\begin{claim}
\label{cl:expfpfp}
In the (FP, FP) subgame, both advertisers will use multipliers of $1$. The revenue of each platform will be $\frac{\alpha^2+1}{2}$.
\end{claim}

\begin{proof}
In this case, since both platforms are symmetric and both running first price auctions, the advertisers will set their multipliers to 1. The query $q^*$ at which advertiser 2 stops winning and advertiser 1 starts winning is thus the one where $\alpha e^{-q^*} = e^{-2q^*}$, or $\alpha = e^{-q^*}$. The revenue is thus $\int_{0}^{q^*} e^{-2q} dq + \int_{q^*}^{\infty} \alpha e^{-q} dq = (-e^{-2q^*}+1)/2 + \alpha e^{-q*} = \alpha^2 + 1/2 - \alpha^2/2 = \frac{1+\alpha^2}{2}$, where we used the fact that $\alpha = e^{-q^*}$.
\end{proof}

\begin{claim}
\label{cl:expspsp}
For $\alpha \in [1/4, 1/2]$, advertiser 1 will use a multiplier of $\mu_1^S = 2$ and advertiser 2 will use a multiplier of $\mu_2^S = \frac{2\alpha}{4\alpha -1}$. The revenue of each platform will be $(3-4\alpha)\alpha$.  
\end{claim}

\begin{proof}
In this case, since the platforms are symmetric, the advertisers will use the same multipliers $\mu_1^S, \mu_2^S$ across both platforms. The efficient $q^*$ is such that 
$$ \mu_1^S \alpha e^{-q^*} = \mu_2^S e^{-2q^*}. $$

In other words $q^*$ is such that $\frac{\mu_1^S \alpha}{\mu_2^S} = e^{-q^*}$. The bidders will use multipliers so that their targets are met. We get the following two equations, one per advertiser:

$$ \int_{q^*}^{\infty} \alpha e^{-q} dq = \int_{q^*}^{\infty} \mu_2^S e^{-2q} dq,$$   

$$ \int_0^{q^*} e^{-2q} dq = \int_0^{q^*} \mu_1^S \alpha e^{-q} dq.$$   

From the first equation, $\alpha e^{-q^*} = \mu_2^S e^{-2q^*}/2$. Therefore, $\mu_2^S = 2 e^{q^*} \alpha$. This combined with the first equation relating $\mu_1^S, \mu_2^S$ implies $\mu_1^S = 2$. From the second equation, let $x = e^{-q^*}$. Rewriting the second equation gives a quadratic equation on $x$. 

$$ (1-x^2)/2 = 2 \alpha (1-x). $$
%{\color{red}[Andres] Simplify since $(1-x^2) = (1-x)(1+x)$ which leads to $x^* = 4 \alpha -1$.}

We manipulate further to get the following. 

$$ 1 - x^2 = 4 \alpha - 4 \alpha x $$
$$ 1-4\alpha = x^2 - 4 \alpha x $$ 
$$ 1-4\alpha + 4 \alpha^2 = x^2 - 4 \alpha x + 4 \alpha^2 $$ 
$$ (1-2\alpha)^2 = (x-2\alpha)^2 $$ 

This only has two sensible solutions. Either the left hand side and the right hand side have the same sign, or they have opposite signs. If they have the same sign, we get that $x = 1$ and $\mu_2^S = 2 \alpha$. This solution only makes sense if $\mu_2^S \geq 1$, i.e. $\alpha > 1/2$. Also $x = 1$ implies $q^* = 0$. We will rule out this case since it will lead to a non-interior allocation, i.e. one advertiser will win all impressions by bidding over the other advertiser. If they don't have the same sign, we get that $x = 4\alpha - 1$. Recall that $x = e^{-q^*}$. Since $q^* \geq 0$, then $0 \leq x \leq 1$. Thus in the other case, we get that $0 \leq 4 \alpha - 1 \leq 1$, or $1/4 \leq \alpha \leq 1/2$ and we get that $\mu_2^S = \frac{2\alpha}{4\alpha-1}$. This proves Claim~\ref{cl:expalpha}.  

Then the revenue can be written as 

$$ \int_0^{q^*} \mu_1^S \alpha e^{-q} dq + \int_{q^*}^{\infty} \mu_2^S e^{-2q} dq $$ 
$$ 2 \alpha (1-e^{-q^*}) + \mu_2^S (e^{-2q^*})/2$$

%If $x=1$, 
%$$ 2 \alpha(1-1) + 2\alpha(1)/2 = \alpha. $$

Because $x=4\alpha-1$, this is the same as 
$$ 2\alpha (1-x) + \left(\frac{2\alpha}{x} x^2\right)/2 = 2 \alpha - \alpha x = \alpha(2-x) = \alpha(3-4\alpha).$$ 
\end{proof}

For the remaining subgame we are able to find the equations that uniquely determine the equilibrium multipliers, but we are not able to write them in a simple closed form.  

%The revenue will depend on the value of $\alpha$, but it can be elegantly written as $\max \{\alpha, (3-4\alpha)\alpha\}$. This is because at $\alpha = 1/2$ both expressions match. For $\alpha > 1/2$, the first term is always greater, for $1/4 < \alpha < 1/2$, the second term is always greater. 

\begin{claim}
\label{cl:expfpsp}
In the (FP, SP) subgame, we present the system of equations that pins down the value of all multipliers and express the overall revenue of each platform as a function of these multipliers and $\alpha$. 
\end{claim}

\begin{proof}
In this case we need four multipliers: $\mu_1^F, \mu_1^S, \mu_2^F, \mu_2^S$, one for each advertiser, platform pair. The index denotes the advertiser, the exponent denotes whether it is the first price (F) or second price (S) platform. The elasticity of the valuations are $\nu_1(q) = |\frac{-\alpha e^{-q}}{\alpha e^{-q}}|=1$, $\nu_2(q) = |\frac{-2 e^{-2q}}{e^{-2q}}| = 2$.

From Eqs.\eqref{eq:intrabidder1}-\eqref{eq:tcpa-final-spa-fpa} we get that 

\begin{align}
\frac{\mu_1^S}{\mu_1^F} &= 1+\frac{1+2}{\alpha e^{-q^F}} \int_{q^F}^{\infty} \alpha e^{-q} dq = 4. \label{eq:expintra1} \\ 
\frac{\mu_2^S}{\mu_2^F} &= 1 + \frac{1+2}{e^{-2q^F}} \int_{0}^{q^F} e^{-2q} dq = 1 + \frac{3}{2} \frac{(1-e^{-2q^F})}{e^{-2q^F}}. \label{eq:expintra2} 
\end{align}

From Eqs.~\ref{eq:tcpa-final-spa-fpa-2},~\ref{eq:tcpa-final-spa-fpa} we get that 

\begin{align} 
(\mu_1^F-1) \alpha e^{-q^F} &= \int_{q_S}^{\infty} (\alpha e^{-q} - \mu_2^S e^{-2q} ) dq = \alpha e^{-q^S} - \mu_2^S e^{-2q^S}/2. \label{eq:exptarget1}\\ 
(\mu_2^F-1) (1- e^{-2q^F})/2 &= \int_{0}^{q^S} (e^{-2q} - \alpha \mu_1^S e^{-q}) dq = (1-e^{-2q^S})/2 - \mu_1^S \alpha(1- e^{-q^S}). \label{eq:exptarget2}
\end{align}

The equilibrium condition necessitates that 

\begin{align}
    \mu_1^F \alpha e^{-q^F} &= \mu_2^F e^{-2q^F}, \label{eq:exfp} \\
    \mu_1^S \alpha e^{-q^S} &= \mu_2^S e^{-2q^S}. \label{eq:expsp}
\end{align}

Therefore, we get equations relating $e^{-q^F}, e^{-q^S}$ to the multipliers. We plug these relations on the set of equations above, and also make the following substitution for legibility $\mu_1^S = x, \mu_1^F = y, \mu_2^S = z, \mu_2^F = w$.


\begin{align}
\frac{x}{y} &= 4 \label{eq:fpsp1}\\
\frac{z}{w} &= 1 + \frac{3}{2} \frac{(1-\frac{y^2 \alpha^2}{w^2})}{\frac{y^2 \alpha^2}{w^2}} \label{eq:fpsp2}\\
(y-1) \frac{\alpha^2 y}{w} &= \alpha^2 \frac{x}{z} - \frac{z \frac{x^2 \alpha^2}{z^2} }{2} \label{eq:fpsp3}\\ 
(w-1)(1-\frac{y^2 \alpha^2}{w^2})/2 &= (1-\frac{x^2\alpha^2}{z^2})/2 - x \alpha (1- \frac{x \alpha}{z}) \label{eq:fpsp4}
\end{align}

We additionally are only interested in equilibria where $x, z \geq 1$ since lower mulitpliers on the second price platform are weakly dominated.  

The revenue for the FP platform is 

$$ \int_{0}^{q^F} \mu_2^F e^{-2q} dq + \int_{q^F}^{\infty} \mu_1^F \alpha e^{-q} dq = \mu_2^F (1-e^{-2q^F})/2 + \mu_1^F \alpha e^{-q^F}.$$ 
    
In terms of the variables established above, this is 

$$ w (1-(\frac{y \alpha}{w})^2)/2 + \frac{y^2 \alpha^2}{w}.$$

The revenue of the SP platform is 

$$ \int_{0}^{q^S} \mu_1^S \alpha e^{-q} dq + \int_{q^S}^{\infty} \mu_2^S e^{-2q} dq = \mu_1^S \alpha (1-e^{-q^S}) + \mu_2^S e^{-2q^S}/2.$$ 

In terms of the variables established above, this is 

$$ x \alpha (1-\frac{x \alpha}{z}) + z \frac{x^2 \alpha^2}{2z^2}. $$
\end{proof}

We can now compute the payoff matrix of the platforms' game induced by the advertisers' subgame equilibrium multipliers. Using Claims~\ref{cl:expfpfp},~\ref{cl:expspsp} and~\ref{cl:expfpsp}:

  \begin{table}[h!]
  \centering
    \setlength{\extrarowheight}{8pt}
    \begin{tabular}{cc|c|c|}
      & \multicolumn{1}{c}{} & \multicolumn{2}{c}{Platform 2}\\
      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{SPA}  & \multicolumn{1}{c}{FPA} \\\cline{3-4}
      \multirow{2}*{Platform 1}  & SPA & $\left((3-4\alpha)\alpha, (3-4\alpha)\alpha \right)$ & $( x \alpha -\frac{x^2 \alpha^2}{2z}),  w/2 (1+ \frac{y^2 \alpha^2}{2w})$ \\\cline{3-4}
      & FPA & $( x \alpha -\frac{x^2 \alpha^2}{2z}),  w/2 (1+ \frac{y^2 \alpha^2}{2w})$
      & $(\frac{\alpha^2+1}{2},\frac{\alpha^2+1}{2})$ \\\cline{3-4}
    \end{tabular}
    \caption{Payoff matrix for the platforms' game after solving for the advertisers' subgame equlibrium, for the valuatiosn described in Section~\ref{sec:expvsexp}.}
    \label{table:expgame}
  \end{table}

We now prove that for $\alpha \in [1/4, 1/2]$, SP is a dominant strategy of the game defined by Table~\ref{table:expgame}.  

\begin{proof}[Proof of Theorem~\ref{thm:expequilibria}]
We change the variables and let $t=\frac{y\alpha}{w}$ and $u=\frac{x\alpha}{z}$. Then we have
\begin{align}
\text{\Cref{eq:fpsp1}} &\iff z=\frac{4wt}{u}    
\end{align}
We plug it into Equations~\ref{eq:fpsp2}-\ref{eq:fpsp4}:
\begin{align}
\text{\Cref{eq:fpsp2}} &\iff \frac{z}{w}=1+\frac{3}{2}\cdot \frac{1-t^2}{t^2} \iff u=\frac{8t^3}{3-t^2} \label{eq:proof_exponential_1}\\
\text{\Cref{eq:fpsp3}} &\iff (\frac{wt}{\alpha}-1)\alpha t=\alpha u -\frac{1}{2}zu^2 \iff wt^2-\alpha t=\alpha u -2uwt \iff w=\frac{\alpha(u+t)}{t^2+2ut} \label{eq:proof_exponential_2}\\
\text{\Cref{eq:fpsp4}} &\iff \frac{1}{2}(w-1)(1-t^2) = \frac{1}{2}(1-u^2) - uz(1-u) \\
&\iff (w-1)(1-t^2) = 1-u^2-8wt(1-u)\iff w=\frac{2-u^2-t^2}{1-t^2+8t-8tu} \label{eq:proof_exponential_3}
\end{align}

By Equations \ref{eq:proof_exponential_1}, \ref{eq:proof_exponential_2} and \ref{eq:proof_exponential_3}, we have
\begin{align}
    \alpha=\alpha(t)=\frac{(2-u^2-t^2)(t^2+2ut)}{(1-t^2+8t-8tu)(u+t)}=\frac{(2-(\frac{8t^3}{3-t^2})^2-t^2)(t^2+2t\cdot\frac{8t^3}{3-t^2})}{(1-t^2+8t-8t\cdot\frac{8t^3}{3-t^2})(\frac{8t^3}{3-t^2}+t)}.
\end{align}
Here we write $\alpha(t)$ as a function of $t$. By \Cref{eq:exfp}, $t=\frac{y\alpha}{w}=e^{-q^F}\in (0,1)$. Similarly, by \Cref{eq:expsp}, $u=\frac{x\alpha}{z}=e^{-q_S}\in (0,1)$. By \Cref{eq:proof_exponential_1}, we further have $\frac{8t^3}{3-t^2}<1$, which implies $t<0.7$. One can verify that when $t\in (0, 0.7)$, $\alpha(t)$ is an increasing function on $t$ (see \Cref{fig:proof_exp1}. As $\alpha(t)\in [1/4, 1/2]$, we have that $0.36<t<0.609$.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.35\textwidth]{proof_exp1.png}
    \caption{The function $\alpha(t)$ when $t\in [0, 0.7]$}
    \label{fig:proof_exp1}
\end{figure}

%Wolframalapha link: https://www.wolframalpha.com/input?i=%282-%288*y%5E3%2F%283-y%5E2%29%29%5E2-y%5E2%29%28y%5E2%2B2*y*%288*y%5E3%2F%283-y%5E2%29%29%29%2F%281-y%5E2%2B8*y-8*y*%288*y%5E3%2F%283-y%5E2%29%29%29%2F%28%288*y%5E3%2F%283-y%5E2%29%29%2By%29+for+0%3Cy%3C0.68

To show that SPA is a dominant strategy of the game, it suffices to show that
\begin{enumerate}
    \item $(3-4\alpha)\alpha >w/2 (1-(\frac{y \alpha}{w})^2) + \frac{y^2 \alpha^2}{w}$.
    \item $x \alpha (1-\frac{x \alpha}{z}) + \frac{x^2 \alpha^2}{2z} > \frac{\alpha^2+1}{2}$.
\end{enumerate}

We notice that when $\alpha\in [1/4, 1/2]$, $(3-4\alpha)\alpha \geq \frac{1}{2}$ and $\frac{\alpha^2+1}{2}\leq 5/8$. It's sufficient to show that (after rewriting the inequalities using $t, u$):
\begin{align}
    \frac{1}{2}>\frac{1}{2}w(1+t^2)\iff F_1(t)=\frac{2-(\frac{8t^3}{3-t^2})^2-t^2}{1-t^2+8t-8t\cdot \frac{8t^3}{3-t^2}}-\frac{1}{1+t^2}<0.\\
    4wt(1-\frac{u}{2})>\frac{5}{8}\iff F_2(t)=\frac{4(2-(\frac{8t^3}{3-t^2})^2-t^2)\cdot t\cdot (1-\frac{8t^3}{2(3-t^2)})}{1-t^2+8t-8t\cdot \frac{8t^3}{3-t^2}}-\frac{5}{8}>0.
\end{align}

One can easily verify that $F_2(t)>0>F_1(t)$ when $t\in (0.36, 0.609)$ (see \Cref{fig:proof_exp3} and \Cref{fig:proof_exp2}). Thus SPA is dominant strategy of the game.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.35\textwidth]{proof_exp3.png}
    \caption{$F_1(t)$ when $t\in [0, 0.7]$}
    \label{fig:proof_exp3}
\end{figure}

%Wolframalapha link: https://www.wolframalpha.com/input?i=f%28y%29%3D%282-%288*y%5E3%2F%283-y%5E2%29%29%5E2-y%5E2%29%2F%281-y%5E2%2B8*y-8*%288*y%5E3%2F%283-y%5E2%29%29*y%29-1%2F%281%2By%5E2%29+for+0%3Cy%3C0.7

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.35\textwidth]{proof_exp2.png}
    \caption{$F_2(t)$ when $t\in [0, 0.7]$}
    \label{fig:proof_exp2}
\end{figure}

%Wolframalapha link: https://www.wolframalpha.com/input?i=4*%282-%288*y%5E3%2F%283-y%5E2%29%29%5E2-y%5E2%29*y*%281-%288*y%5E3%2F%283-y%5E2%29%29%2F2%29%2F%281-y%5E2%2B8*y-8*y*%288*y%5E3%2F%283-y%5E2%29%29%29-5%2F8+for+0%3Cy%3C0.7

\end{proof}

\begin{comment}

\subsubsection{Specific choice of $\alpha$}

When $\alpha = .25$: $x = 3.1, z = 6.088, w = .549, y = .790$ and revenues as follows: 

  \begin{table}[h!]
  \centering
    \setlength{\extrarowheight}{8pt}
    \begin{tabular}{cc|c|c|}
      & \multicolumn{1}{c}{} & \multicolumn{2}{c}{Ch 1}\\
      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{SPA}  & \multicolumn{1}{c}{FPA} \\\cline{3-4}
      \multirow{2}*{Ch 2}  & SPA & (.50, .50) & $( .7386 , .310)$ \\\cline{3-4}
      & FPA & $(.310, .7386)$ & $(.531, .531)$ \\\cline{3-4}
    \end{tabular}
    \caption{Table for $\alpha = .25$}
  \end{table}
  
SP is a dominant strategy, hence (SP, SP) is the only equilibrium. 

When $\alpha = 1/3$ - this alpha is interesting because it is when SPA rev and FPA rev match! We get$w =.4925, x = 2.852, y = .713, z = 2.9265$ and revenues as follows: 

  \begin{table}[h!]
  \centering
    \setlength{\extrarowheight}{8pt}
    \begin{tabular}{cc|c|c|}
      & \multicolumn{1}{c}{} & \multicolumn{2}{c}{Ch 1}\\
      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{SPA}  & \multicolumn{1}{c}{FPA} \\\cline{3-4}
      \multirow{2}*{Ch 2}  & SPA & (.5555, .5555) & $( .796 , .303)$ \\\cline{3-4}
      & FPA & $(.303, .796)$ & $(.5555, .5555)$ \\\cline{3-4}
    \end{tabular}
    \caption{Table for $\alpha = 1/3$}
  \end{table}

So in this example, the only equilibrium is (SPA, SPA). SPA is a dominant strategy.

When $\alpha = 3/8$ - this case is interesting because it is the point where SP SP rev is maximized. Here we get that $w = .523, x = 2.808, y = .702, z = 2.837$. For these values, the revenues are like this: 

  \begin{table}[h!]
  \centering
    \setlength{\extrarowheight}{8pt}
    \begin{tabular}{cc|c|c|}
      & \multicolumn{1}{c}{} & \multicolumn{2}{c}{Ch 1}\\
      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{SPA}  & \multicolumn{1}{c}{FPA} \\\cline{3-4}
      \multirow{2}*{Ch 2}  & SPA & (.5625, .5625) & $( .744 , .313)$ \\\cline{3-4}
      & FPA & $(.313, .744)$ & $(.57, .57)$ \\\cline{3-4}
    \end{tabular}
    \caption{Table for $\alpha = 3/8$}
  \end{table}

So in this example, the only equilibrium is (SPA, SPA). SPA is a dominant strategy.

When $\alpha = 1/2$ we get that $w = .536, x = 2.61, y = .653, z = 1.90$. For these values, the revenues are like this:
 
  \begin{table}[h!]
  \centering
    \setlength{\extrarowheight}{8pt}
    \begin{tabular}{cc|c|c|}
      & \multicolumn{1}{c}{} & \multicolumn{2}{c}{Ch 1}\\
      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{SPA}  & \multicolumn{1}{c}{FPA} \\\cline{3-4}
      \multirow{2}*{Ch 2}  & SPA & (1/2, 1/2) & $( .856 , .367)$ \\\cline{3-4}
      & FPA & $(.367, .856)$ & $(5/8, 5/8)$ \\\cline{3-4}
    \end{tabular}
    \caption{Table for $\alpha = 1/2$}
  \end{table}  
  
So in this example, the only equilibrium is (SPA, SPA). SPA is a dominant strategy.
  
When $\alpha = 3/4$ - this is kinda random choice on my part. We get that $w = .715, y = .633, x = 2.53, z = 2.07$.  

 
  \begin{table}[h!]
  \centering
    \setlength{\extrarowheight}{8pt}
    \begin{tabular}{cc|c|c|}
      & \multicolumn{1}{c}{} & \multicolumn{2}{c}{Ch 1}\\
      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{SPA}  & \multicolumn{1}{c}{FPA} \\\cline{3-4}
      \multirow{2}*{Ch 2}  & SPA & (3/4, 3/4) & $( 1.029 , .5151)$ \\\cline{3-4}
      & FPA & $(1.029, .5151)$ & $(.78, .78)$ \\\cline{3-4}
    \end{tabular}
    \caption{Table for $\alpha = 3/4$}
  \end{table}  

So in this example, the only equilibrium is (SPA, SPA). SPA is a dominant strategy.

When $\alpha = 1$, the highest possible value for alpha for us, we get that $w = .924, y = .628, x = 2.51, z = 2.54$.  

 
  \begin{table}[h!]
  \centering
    \setlength{\extrarowheight}{8pt}
    \begin{tabular}{cc|c|c|}
      & \multicolumn{1}{c}{} & \multicolumn{2}{c}{Ch 1}\\
      & \multicolumn{1}{c}{} & \multicolumn{1}{c}{SPA}  & \multicolumn{1}{c}{FPA} \\\cline{3-4}
      \multirow{2}*{Ch 2}  & SPA & (1,1) & $( 1.2727, .675)$ \\\cline{3-4}
      & FPA & $(.675, 1.2727)$ & $(1, 1)$ \\\cline{3-4}
    \end{tabular}
    \caption{Table for $\alpha = 1$}
  \end{table}  

So in this example, the only equilibrium is (SPA, SPA). SPA is a dominant strategy.
\end{comment}

\begin{comment}
\section{Study Case 3: Linear vs Linear}

Here we consider $v_1(q) = \alpha q, v_2(q) = \beta(1-q)$. 

\subsection{Sub game 1: First Price, First Price}

In this case, the multipliers are both $1$. Here the efficient $q^* = \frac{\beta}{\alpha+\beta}$. The revenue for each platform (since it is symmetric) is 

\begin{align*}
\int_{0}^{q^*} (1-q) \beta dq = \int_{q^*}^{1} \alpha q dq & = \beta (q^*-{q^*}^2/2) + \alpha (1-{q^*}^2)/2 \\ 
\beta \frac{\beta}{(\alpha+\beta)} \left(1-\frac{\beta}{2(\alpha+\beta)}\right) + \frac{\alpha}{2} \frac{\alpha}{(\alpha+\beta)} \frac{\alpha + 2\beta}{(\alpha+\beta)} & = \frac{\beta^2 (2\alpha+\beta)}{2(\alpha+\beta)^2} + \frac{\alpha^2 (\alpha+2\beta)}{2(\alpha+\beta)^2}\\
\frac{(\alpha+\beta)^3 - \alpha \beta (\alpha+\beta)}{2(\alpha+\beta)^2} & = \frac{(\alpha+\beta)^2-\alpha \beta}{2(\alpha+\beta)} \\
\end{align*}

So this is the revenue for either platform. Note if $\alpha = \beta = 1$, then the revenue is $3/4$, which makes sense. 

\subsection{Sub game 2: Second Price, Second Price}

In this case, since the platforms are symmetric, the multipliers for each platform will be the same so we'll just look for $\mu_1,\mu_2$. The efficient allocation satisfies

\begin{align*}
    \mu_1 q^* \alpha &= \mu_2 \beta (1-q^*) \\
    q^* &= \frac{\mu_2 \beta}{\mu_2 \beta + \mu_1 \alpha} \\
\end{align*}

The platforms will set multipliers so as to match value to their spend

\begin{align*}
    \int_{q^*}^{1} \alpha q dq & =  \int_{q^*}^{1} \beta \mu_2 (1-q) dq \\ 
    \int_{0}^{q^*} \beta (1-q) dq & = \int_{0}^{q^*} \alpha \mu_1 q dq \\
\end{align*}

Solving this out gives
\begin{align*}
    \beta (1-q^*/2) = \alpha \mu_1 q^*/2  \\ 
    \alpha(1+q^*) = \beta \mu_2 (1-q^*) \\ 
\end{align*}

Therefore we get 
\begin{align*}
    \mu_1 = \frac{2 \beta (1-q^*/2)}{\alpha q^*} \\
    \mu_2 = \frac{\alpha (1+q^*)}{\beta (1-q^*)} \\
\end{align*}

Plugging in $q^*$, we get 

\begin{align*}
    2(\mu_1\alpha + \mu_2 \beta) = \mu_2(\mu_1\alpha+\beta)\\ 
    2\mu_2 \beta + \mu_1 \alpha = \mu_2 \beta \mu_1 \\ 
\end{align*}

At least for $\alpha = \beta$ all this gives $q^* = 1/2$ (as expected) and $\mu_1 = \mu_2 = 3$.

Solving for $\mu_1, \mu_2$ gives 

\begin{align*}
    \mu_1 = \frac{\beta (4-\alpha)}{2-\alpha} \\ 
    \mu_2 = \frac{4-\alpha}{2 \alpha - \beta} \\ 
\end{align*}

This gives some conditions, $\alpha < 4, 2\beta > \alpha^2, 2\alpha > \beta$. 

The revenue for each platform would be 

\begin{align*}
\int_{0}^{q^*} \mu_1 \alpha q \dq + \int_{q^*}^{1} \mu_2 \beta (1-q) dq & = \\
\mu_1 \alpha (q^*)^2 + \mu_2 \beta (1-q^*)^2/2 & \\ 
\end{align*}

\subsection{Sub game 3: First Price, Second Price}

Let $\mu_1^S = x, \mu_1^F =y, \mu_2^S = z, \mu_2^F = w, q_F = F, q_S = S$. Then the equations governing this game are 

\begin{align*}
    \frac{x}{y} &= 1 + \frac{(1+F)}{2F^2} \\
    \frac{z}{w} &= 1 + \frac{(2-F)}{2(1-F^2)} \\ 
    (y-1)(1-F^2) \alpha &= \alpha (1-S^2) - z \beta (1-S)^2 \\ 
    (w-1) \beta F (2-F) &= \beta S (2-S) - x\alpha S^2 \\
    F &= \frac{\beta w}{\beta w + \alpha y} \\ 
    S &= \frac{\beta z}{\beta z + \alpha x} \\ 
\end{align*}

\end{comment}
